Tamper Detection against Unitary Operators

Security of a storage device against a tampering adversary has been a well-studied topic in classical cryptography. Such models give black-box access to an adversary, and the aim is to protect the stored message or abort the protocol if there is any tampering. In this work, we extend the scope of the theory of tamper detection codes against an adversary with quantum capabilities. We consider encoding and decoding schemes that are used to encode a $k$-qubit quantum message $\vert m\rangle$ to obtain an $n$-qubit quantum codeword $\vert {\psi_m} \rangle$. A quantum codeword $\vert {\psi_m} \rangle$ can be adversarially tampered via a unitary $U$ from some known tampering unitary family $\mathcal{U}_{\mathsf{Adv}}$ (acting on $\mathbb{C}^{2^n}$). Firstly, we initiate the general study of \emph{quantum tamper detection codes}, which detect if there is any tampering caused by the action of a unitary operator. In case there was no tampering, we would like to output the original message. We show that quantum tamper detection codes exist for any family of unitary operators $\mathcal{U}_{\mathsf{Adv}}$, such that $\vert\mathcal{U}_{\mathsf{Adv}} \vert < 2^{2^{\alpha n}}$ for some constant $\alpha \in (0,1/6)$; provided that unitary operators are not too close to the identity operator. Quantum tamper detection codes that we construct can be considered to be quantum variants of \emph{classical tamper detection codes} studied by Jafargholi and Wichs~['15], which are also known to exist under similar restrictions. Additionally, we show that when the message set $\mathcal{M}$ is classical, such a construction can be realized as a \emph{non-malleable code} against any $\mathcal{U}_{\mathsf{Adv}}$ of size up to $2^{2^{\alpha n}}$.

==> TD/Classical_TD_Backedup.tex <==
\section{A Warm-up: Quantum tamper detection codes for classical messages}\label{cqtdc}
In this section, we consider quantum tamper detection codes for classical messages. We give a probabilistic proof that quantum tamper detection codes for classical messages exist.
%\subsection{A Probabilistic Method Approach}
\begin{theorem}\label{mainthm}
Let $\mathcal{U}_{\mathsf{Adv}}$ be an $\left(N,\alpha, \sqrt{\frac{\eps}{2K}}\right)$ family such that $ \left( \frac{1}{6} - \alpha\right) \log(N)  \geq \log(K) + \log\left( \frac{1}{\eps}\right)+ 5$.
Then there exists a $(K, N, \eps)$-tamper secure scheme for classical messages.
Furthermore, a uniformly random encoding and decoding strategy according to Haar measure \emph{(}see $(\enc, \dec_{\mathsf{Cl}})$ in Definition~\ref{def:random_haar_enc_dec}\emph{)} gives such a code with probability at least $1-  \mathcal{O} \left(\dfrac{K^2 N}{ 2^{N^{\alpha}}}\right)$. 
\end{theorem}
\begin{proof}	
	We show that an encoding and decoding strategy, as given in Definition~\ref{def:random_haar_enc_dec}, gives a tamper detection code for the given set of parameters. 

	For a fixed unitary $U \in \mathcal{U}_{\mathsf{Adv}}$, let us define random variables $X_{js} = \vert \bra{\psi_j}U\ket{\psi_s}\vert^2$  {for $j,s \in \mathcal{M}$}.
	 Here the randomness is over the Haar measure in choosing $(\enc, \dec )$ strategy as an isometry $V$.
	 Let $X_s = \sum_{j \ne s}  X_{js}.$ 
	 The random variable $X_{js}$ denotes the probability that message $j$ was decoded given that message $s$ was encoded.
	 Similarly, $X_s$ denotes the probability that the procedure resulted in an incorrectly decoded message.  
	 Both $X_{js}$ and $X_s$ are non-negative random variables with values less than or equal to $ 1$.
	 
	Let $\clE$ be the event that  $(\enc, \dec)$  is not an $\eps$-secure tamper detection code against  $\mathcal{U}_{\mathsf{Adv}}$. Then, 	
	\begin{align*}
		\Pr\left(\clE   \right) & \leq \Pr\left(   \exists  U \in \mathcal{U}_{\mathsf{Adv}}, s \in \{ 0,1 \}^k  \quad \text{s.t.}  \quad X_s+X_{ss} \geq \eps \right)\\
		& \leq \sum_{ U \in \mathcal{U}_{\mathsf{Adv}}} \sum_{s \in \{ 0,1 \}^k} \Pr\left(  X_s +X_{ss}  \geq \eps  \right)  \\
		& \leq \sum_{ U \in \mathcal{U}_{\mathsf{Adv}}} \sum_{s \in \{ 0,1 \}^k} \sum_{j \in \{ 0,1 \}^k \ne s}  \Pr\left(  X_{js}  \geq \frac{\eps}{K}   \right) +\sum_{ U \in \mathcal{U}_{\mathsf{Adv}}} \sum_{s \in \{ 0,1 \}^k} \Pr\left(  X_{ss}  \geq \frac{\eps}{K}  \right)  \\
		& \leq  \vert \mathcal{U}_{\mathsf{Adv}} \vert K^2 \Pr\left( X_{js}  \geq \frac{\eps}{K}   \right) + \vert \mathcal{U}_{\mathsf{Adv}} \vert K \Pr\left(  X_{ss}  \geq \frac{\eps}{K}    \right) \\
		& =  \vert \mathcal{U}_{\mathsf{Adv}} \vert K^2 	\Pr\left(\clE_1   \right) + \vert \mathcal{U}_{\mathsf{Adv}} \vert K 	\Pr\left(\clE_2   \right). \\
	\end{align*}
	To bound  $\Pr\left(\clE_1   \right)=\Pr\left(  X_{js}  \geq \frac{\eps}{K}   \right) $ and  $\Pr\left(\clE_2   \right)=\Pr\left(  X_{ss}  \geq  \frac{\eps}{K}   \right)$ using a Chernoff-like argument, we need to calculate moments of random variable $X_{js}$ and $X_{ss}$.	
	Note that we could not directly use Chernoff bound to bound $\sum_j X_{js}$ as for different $j_1 \neq j_2$, the random variables $X_{j_{1}s}$ and $X_{j_{2}s}$ are not independent of each other.
	Naturally, the problem of calculating moments of random variable $X_{js}$ is closely related to Weingarten unitary calculus (see Section~\ref{wuc}) as our encoding strategy is Haar random.

Here we present first-order moments for variables $X_{js}$ and $X_{ss}$. 
Computation for higher moments is similar but slightly more involved and can be found in the Appendix~\ref{sec:app_classical}.

For readability we use $\phi = \sqrt{\frac{\eps}{2K}}$. 
Thus, $\mathcal{U}_{\mathsf{Adv}}$ is an $(N, \alpha, \phi)$ family.

\vspace{0.4cm}
 
	\textbf{First moment of random variable $X_{js}$ and $X_{ss}$:} 
	
	We begin with the first moment of $X_{js}$. 
	\begin{align*}
		X_{js} & = |\bra{\psi_j}U\ket{\psi_s}|^2\\
		& = \bra{\psi_j}U\ket{\psi_s}\bra{\psi_s}U^\dagger \ket{\psi_j} \\
		& = \bra{j}V^\dagger UV\ket{s}\bra{s}V^\dagger U^\dagger V\ket{j} \\
		& = \left(\sum_{l_1,k_1}U_{l_1k_1} V^*_{l_1j}V_{k_1s}\right) \left(\sum_{l_2 ,k_2}U^\dagger_{l_2k_2} V^*_{l_2s}V_{k_2j} \right) \\
		& = \sum_{l_1,k_1}\sum_{l_2,k_2}\left(U_{l_1k_1} U^\dagger_{l_2k_2} V_{k_1s}V_{k_2j} V^*_{l_1j}V^*_{l_2s}\right).
	\end{align*}
	
	\noindent\textbf{A.} When $j \ne s$,
	\begin{align*}
		\E[X_{js}]& = \E[|\bra{\psi_j}U\ket{\psi_s}|^2]\\
		& = \sum_{l_1,k_1}\sum_{l_2,k_2}\left(U_{l_1k_1} U^\dagger_{l_2k_2} \E\left[V_{k_1s}V_{k_2j} V^*_{l_1j}V^*_{l_2s}\right]\right) \\ 
		& = \sum_{l_1,k_1}\sum_{l_2,k_2}\left(U_{l_1k_1} U^\dagger_{l_2k_2}   \left( \sum_{\alpha, \beta \in S_2} \delta_{\alpha}(k_1k_2,l_1l_2)\delta_{\beta}(sj,js) \wg(\beta \alpha^{-1},N)\right) \right).
	\end{align*} 
	The final equality is due to Fact~\ref{wgt}.
	Note that when $j \ne s$ and $\beta= \id$, we get, $\delta_{\beta}(sj,js) =0$.
	Thus, the only terms that survive are those corresponding to $\beta= \left(1 \ 2 \right)$. 
	
	\begin{align*}
		\E[X_{js}]& = \sum_{l_1,k_1,l_2,k_2}U_{l_1k_1} U^\dagger_{l_2k_2}   \left( \delta(k_1k_2,l_1l_2) \wg((1\ 2) ((1)(2))^{-1},N) + \delta(k_1k_2,l_2l_1) \wg((1\ 2) (1\ 2)^{-1},N)  \right)\\
		& = \sum_{l_1=k_1}\sum_{l_2=k_2}U_{l_1k_1} U^\dagger_{l_2k_2}  \wg((1\ 2),N) +   \sum_{l_1=k_2}\sum_{l_2=k_1}U_{l_1k_1} U^\dagger_{l_2k_2} \wg((1)(2),N)  \\ 
		& = \Tr(U)  \Tr(U^\dagger)\cdot \wg((1\ 2),N) +   \Tr(UU^\dagger) \cdot \wg((1)(2),N)  \\ 
		& =\frac{- \Tr(U)  \Tr(U^\dagger) }{N(N^2-1)}+  N \cdot \frac{1}{N^2-1} \\ 
		& =\frac{ N^2- \Tr(U)  \Tr(U^\dagger) }{N(N^2-1)}\\ 
		& =\frac{ N^2- \vert\Tr(U)\vert^2  }{N(N^2-1)}\\ 
		& \leq \frac{ 2 }{N} \;.
	\end{align*}


 
 \noindent \textbf{B.} When $j = s$,
	\begin{align*}
		\E[X_{ss}]& = \E[|\bra{\psi_s}U\ket{\psi_s}|^2] \nonumber \\
		& = \sum_{l_1,k_1}\sum_{l_2,k_2}\left(U_{l_1k_1} U^\dagger_{l_2k_2} \E\left[V_{k_1s}V_{k_2s} V^*_{l_1s}V^*_{l_2s}\right]\right) \nonumber \\ 
		& = \sum_{l_1,k_1}\sum_{l_2,k_2}\left(U_{l_1k_1} U^\dagger_{l_2k_2}   \left( \sum_{\alpha, \beta \in S_2} \delta_{\alpha}(k_1k_2,l_1l_2)\delta_{\beta}(ss,ss) \wg(\beta \alpha^{-1},N)\right) \right) & (\mbox{from Fact~\ref{wgt}}) \\ 
		& =  \sum_{\alpha \in S_2} \left(\sum_{l_1,k_1,l_2,k_2}U_{l_1k_1} U^\dagger_{l_2k_2}    \delta_{\alpha}(k_1k_2,l_1l_2) \left(\sum_{\beta \in S_2}\wg(\beta \alpha^{-1},N)\right) \right) \nonumber \\
		& =  \sum_{\alpha \in S_2} \left(\sum_{l_1,k_1,l_2,k_2}U_{l_1k_1} U^\dagger_{l_2k_2}    \delta_{\alpha}(k_1k_2,l_1l_2) \left( \frac{1}{N(N+1)}\right) \right)& (\mbox{from Eq.~\eqref{wg_sum}}) \\
		& = \frac{1}{N(N+1)}\left(\sum_{l_1=k_1}\sum_{l_2=k_2}U_{l_1k_1} U^\dagger_{l_2k_2}  +   \sum_{l_1=k_2}\sum_{l_2=k_1}U_{l_1k_1} U^\dagger_{l_2k_2}\right) \nonumber  \\ 
		& = \frac{\Tr(U)  \Tr(U^\dagger) +   \Tr(UU^\dagger) }{N(N+1)}  \\ 
			& =  \frac{ N+ \vert \Tr(U)\vert^2 }{N(N+1)} \nonumber \leq \phi^2 + \frac{1}{N} & (\mbox{since $\vert\Tr(U) \vert \leq \phi N$}).
	\end{align*}

Thus, we get the following bounds:
\begin{gather*}
     \E\left[X_{js}\right] \leq \frac{2}{N} \quad  and \quad 
    \E[X_{ss}] \leq \phi^2+ \frac{1}{N} \;.
\end{gather*}

Similarly, we get higher moment bounds (see Appendix~\ref{sec:app_classical});
\begin{gather}
    \E\left[X_{js}^{t}\right] \leq\mathcal{O}\left( \frac{t^4}{N}\right)
^t \quad and \quad \E[X_{ss}^{t}] \leq \mathcal{O}{\left( \left( \frac{t^2}{N}\right)^t + t \phi^{2t} \right)}. \label{claim:t-moments_classical}   \end{gather}


Now we proceed to bound the probability $ \Pr\left(  X_{js}  \geq  \frac{\eps }{K}  \right).$
	\begin{align}
		\Pr\left(  X_{js}  \geq  \frac{\eps }{K}   \right) & \leq \Pr\left(  e^{ \theta X_{js}}  \geq e^{ \frac{\theta \eps }{K}   }  \right) \nonumber  \\
		& \leq \frac{\E[  e^{ \theta X_{js}} ] }{e^{ \frac{\theta \eps }{K}  }  } \nonumber  \\
		& =  \frac{ 1 }{e^{ \frac{\theta \eps }{K}  } }  \sum_i  \frac{ \theta^i \E[X_{js}^i]}{i! } \nonumber  \\
		& = \frac{ 1 }{e^{ \frac{\theta \eps }{K}  } }  \left( \sum_{i=0}^{N^{1/5}}  \frac{\theta^i   \E( X_{js}^i)}{i! }+  \sum_{i \geq N^{1/5}+1} \frac{ \theta^i  \E(  X_{js}^i)}{i! }\right) \nonumber  \\
		& \leq \frac{ 1 }{e^{ \frac{\theta \eps }{K}    } } \left( \sum_{i=0}^{N^{1/5}}  \frac{ \theta^i}{i! } \clO \left(\frac{ i^4 }{N }\right)^i+  \sum_{i \geq N^{1/5}+1} \frac{\theta^i  \E(X_{js}^i)}{i! }\right)   & \tab (\mbox{from Eq.~\eqref{claim:t-moments_classical}}) \nonumber \\
		& \leq \frac{ 1 }{e^{ \frac{\theta \eps }{K}  } } \left( \sum_{i=0}^{N^{1/5}}  \frac{ 1}{i! } \clO \left(\frac{ \theta}{N^{1/5} }\right)^i+  \sum_{i \geq N^{1/5}+1} \frac{\theta^i  \E(X_{js}^i)}{i! }\right) \nonumber  \\
		& \leq \frac{ 1 }{e^{ \frac{\theta \eps }{K} } } \left( \sum_{i=0}^{N^{1/5}}  \frac{ 1}{i! } \clO \left(\frac{ \theta}{N^{1/5} }\right)^i+  \sum_{i \geq N^{1/5}+1} \frac{\theta^i  \E(  X_{js}^{N^{1/5}})}{i! }\right) \nonumber  \\
		& \leq    \frac{ 1 }{e^{ \frac{\theta \eps }{K}  } }  \left( \clO \left(e^{ \frac{\theta}{N^{1/5}}} \right)+  \clO \left(\frac{e^\theta}{ N^{\frac{1}{5}N^{1/5}}  }\right)\right) \nonumber  \\
		& \leq    \frac{ 1 }{e^{ \frac{\theta \eps }{K} } } \clO \left( e^{ \frac{\theta}{N^{1/5}}} +  e^{\theta - \frac{1}{5}N^{1/5} \ln(N)  } \right) \nonumber  \\
		\label{jsboundeq10}& \leq  \clO \left( e^{ \frac{\theta}{N^{1/5}} -  \frac{\theta \eps }{K}  }  +  e^{\theta - \frac{\theta \eps }{K}   - \frac{1}{5}N^{1/5} \ln(N)  } \right).
	\end{align} 
	
	Similarly when $j=s$, we bound the probability $ \Pr\left(  X_{ss} \geq \frac{\eps}{K}  \right).$
	\begin{align}
		\Pr\left(  X_{ss}  \geq  \frac{\eps }{K}   \right) & \leq \Pr\left(  e^{ \theta X_{ss}}  \geq e^{ \frac{\theta \eps }{K}   }  \right) \nonumber  \\
		& \leq \frac{\E[  e^{ \theta X_{ss}} ] }{e^{ \frac{\theta \eps }{K}  }  } \nonumber  \\
		& =  \frac{ 1 }{e^{ \frac{\theta \eps }{K}  } }  \sum_i  \frac{ \theta^i \E[X_{ss}^i]}{i! } \nonumber  \\
		& = \frac{ 1 }{e^{ \frac{\theta \eps }{K}  } }  \left( \sum_{i=0}^{N^{1/5}}  \frac{\theta^i   \E( X_{ss}^i)}{i! }+  \sum_{i \geq N^{1/5}+1} \frac{ \theta^i  \E(  X_{ss}^i)}{i! }\right) \nonumber  \\
		& \leq \frac{ 1 }{e^{ \frac{\theta \eps }{K}    } }\  \clO\left( \sum_{i=0}^{N^{1/5}}  \frac{ \theta^i}{i! } \left( i\phi^{2i}  + \left( \frac{1}{N^{3/5}} \right)^i\right)+  \sum_{i \geq N^{1/5}+1} \frac{\theta^i  \E(X_{ss}^i)}{i! }\right) \hspace{1.236cm} 
  \\ & \omit\hfill (\mbox{from Eq.~\eqref{claim:t-moments_classical}}) \nonumber \\
		& \leq \frac{ 1 }{e^{ \frac{\theta \eps }{K}  } }\  \clO \left( N\sum_{i=0}^{N^{1/5}}  \frac{ (\theta\phi^{2})^i}{i! } +  \sum_{i=0}^{N^{1/5}}    \frac{ 1}{i! }   \left( \frac{\theta}{N^{3/5}} \right)^i  +    \left(\left(  \frac{1}{N^{3/5}}   \right)^{N^{1/5}}  + N \phi^{N^{1/5}}   \right) e^{\theta }\right) \nonumber  \\
		\label{sstboundeq111}& \leq   \frac{ 1 }{e^{ \frac{\theta \eps }{K}  } }\ \clO\left(   N e^{\theta\phi^{2}} + e^{ \frac{\theta}{N^{3/5}}} +  e^{\theta   - \frac{3}{5} N^{1/5} \ln(N)  } + e^{\theta +\ln(N)   -N^{1/5} \ln(1/\phi)  } \right).
	\end{align} 
	
	Choosing $\theta  = N^{\frac{1}{6}}$, we have, 
	\begin{flalign}
	& \vert\mathcal{U}_{\mathsf{Adv}} \vert  K^2\Pr\left(\clE_1   \right)  = 	\vert\mathcal{U}_{\mathsf{Adv}} \vert K^2 \Pr\left(  X_{js}  \geq \frac{\eps}{K}   \right) \nonumber \\
		& \leq  	\vert\mathcal{U}_{\mathsf{Adv}} \vert K^2   \Pr\left(  e^{ \theta X_{js}}  \geq e^{ \frac{\theta \eps }{K}   }  \right) \nonumber \\
		& \leq  \vert\mathcal{U}_{\mathsf{Adv}} \vert K^2\ \clO\left( e^{ \frac{\theta}{N^{1/5}} -  \frac{\theta \eps }{K}  }  +  e^{\theta - \frac{\theta \eps }{K} - \frac{1}{5} N^{1/5} \ln(N)  } \right) \hspace{5.6cm} (\mbox{from Eq.~\eqref{jsboundeq10}}) \nonumber\\
		& \leq  2^{2^{\alpha n}} K ^2   \mathcal{O}\left(2^{   2^{n/6 - n/5} \log(e)- \log(e)  2^{n/6 -\lambda-k}} + 2^{  2^{n/6} \log(e)- \log(e) 2^{n/6-\lambda-k} -\frac{n}{5} 2^{n/5} \frac{1}{\log e}} \right)   \nonumber \\
		& \leq K^2  \mathcal{O}\left(2^{  2^{\alpha n}+   1- 2 \cdot 2^{\alpha n} } + 2^{  2^{\alpha n}+    2^{n/6} \log(e)- 2\cdot 2^{\alpha n}  -n 2^{n/5} \frac{1}{\log e}}\right) \nonumber   \\
		& \leq K^2 \mathcal{O}\left(  2^{  -2^{\alpha n}+  1 } + 2^{  -2^{\alpha n}+   1} \right) \hspace{4.2cm}    \nonumber  \\
		\label{e1eq4}& \leq \mathcal{O}\left(\dfrac{K^2 N}{ 2^{N^{\alpha}}}\right). 
	\end{flalign}
	The last three inequalities follow from the choice of our parameters; 
	\[ \left( \frac{1}{6} - \alpha\right) \log(N)  \geq \log(K) + \log\left( \frac{1}{\eps}\right)+ 5 \tab \text{and} \tab  \eps = 2^{-
 \lambda}.\] 
	
	
    Similarly, we have, 
	\begin{align}
		& \vert \mathcal{U}_{\mathsf{Adv}} \vert K \Pr\left(\clE_2   \right)  = \vert \mathcal{U}_{\mathsf{Adv}} \vert K \Pr\left(  X_{ss}  \geq \frac{\eps}{K}   \right) \nonumber \\
		& \leq \vert \mathcal{U}_{\mathsf{Adv}} \vert K   \Pr\left(  e^{ \theta X_{ss}}  \geq e^{ \frac{\theta \eps }{K}   }  \right) \nonumber \\
		\nonumber & \leq \vert \mathcal{U}_{\mathsf{Adv}} \vert K    \frac{ 1 }{e^{ \frac{\theta \eps }{K}  } } \clO \left(   N e^{\theta\phi^{2}} + e^{ \frac{\theta}{N^{3/5}}} +  e^{\theta   - \frac{3}{5} N^{1/5} \ln(N)  } + e^{\theta +\ln(N)   -N^{1/5} \ln(1/\phi)  } \right) \tab (\mbox{from Eq.~\eqref{sstboundeq111}}) \\
		& \leq \mathcal{O}\left(2^{  2^{\alpha n}+ k-  2^{n/6-\lambda-k}  \log(e) } \left( 2^{  n+  2^{n/6} \phi^2 \log(e) } + 2^{ 2^{n/6-3n/5}  \log(e) } +2^{  2^{n/6}\log(e) -\frac{3}{5} 2^{n/5}\log(e)} + 2^{  2^{n/6}\log(e)+n - 2^{n/5}\log(\frac{1}{\phi})} \right) \right)  \nonumber \\
	    & \leq  \mathcal{O}\left(2^{  -2^{\alpha n}+ k+n+ 1 } + 2^{  -2^{\alpha n}+ k+  1} + 2^{  -2^{\alpha n}+ k+  1} + 2^{  -2^{\alpha n}+ k+ n+ 1} \right) \nonumber \\
		\label{e2eq4}& \leq   \mathcal{O} \left(\dfrac{K^2 N}{ 2^{N^{\alpha}}}\right). 
	\end{align}
Last three inequalities follows from our choice of parameters; since $\phi= \sqrt{\frac{\eps}{4K}}$ and $ \left( \frac{1}{6} - \alpha\right) \log(N)  \geq \log(K) + \log\left( \frac{1}{\eps}\right)+ 5$.
Thus, it follows from Eqs~\eqref{e1eq4}~and~\eqref{e2eq4} that
\begin{align*}
	\Pr\left(\clE   \right) & \leq  \vert \mathcal{U}_{\mathsf{Adv}} \vert K^2 	\Pr\left(\clE_1   \right) + \vert \mathcal{U}_{\mathsf{Adv}} \vert K 	\Pr\left(\clE_2   \right) \leq  \mathcal{O} \left(\dfrac{K^2 N}{ 2^{N^{\alpha}}}\right). \qedhere
\end{align*}
\end{proof}
\subsection{Relaxed tamper detection for classical messages}\label{Sec:Relaxed_TD}
We would like to point out that an interesting side result follows from our previous calculation. 
It follows that one can get a \emph{relaxed} version of tamper detection even if even when the family $\mathcal{U}_{\mathsf{Adv}}$ does not satisfy the \emph{far from identity} condition. 
Recall that, in the relaxed version, we aim to either output the original message or detect that it was tampered and output $\perp$.
In principle, the relaxed version allows us to revert back to the original message without detecting tampering. 
Such a ``reversion without detection" is inherent to the quantum setting due to the action of measurement operators.
For example, consider a message $m$ encoded as $\ket{\psi}$.
Suppose a unitary takes $\ket{\psi}$ to $\frac{1}{\sqrt{2}} \left( \ket{\psi} + \ket{\psi^\prime}\right)$ where $\ket{\psi^\prime}$ is orthogonal to the space of codewords.  The measurement of the decoder can result in $\ket{\psi^\prime}$ indicating that there was tampering.
If the measurement results in $\ket{\psi}$, we can not detect the tampering, but nonetheless, the decoder still outputs the correct message $\widehat{m}=m$. 
Thus, one gets a qualitatively similar version of tamper detection where the decoder either aborts or returns the correct plaintext.
\begin{theorem}\label{thm:relaxedclassical}
    Let $\mathcal{U}_{\mathsf{Adv}}$ be an $\left(N, \alpha, 1\right)$ family such that $ \left( \frac{1}{6} - \alpha\right) \log(N)  \geq \log(K) + \log\left( \frac{1}{\eps}\right)+ 5$. Then a uniform Haar random encoding-decoding strategy is $(K,N,\eps)$-relaxed tamper secure with probability at least $1-  \mathcal{O} \left(\dfrac{K^2 N}{2^{N^{\alpha}}}\right)$.
\end{theorem}
\begin{proof}For a fixed unitary $U$, recall that random variables were defined as follows: $X_{js} = |\bra{\psi_j}U\ket{\psi_s}|^2$ and $X_s = \sum\limits_{j \ne s}  X_{js}.$ Let $\clE$ be the event that  $(\enc, \dec)$  is not an $\eps$-secure relaxed tamper detection code against  $\mathcal{U}_{\mathsf{Adv}}$.
   \begin{align*}
			\Pr\left(\clE   \right) & \leq \Pr\left(   \exists  U \in \mathcal{U}_{\mathsf{Adv}}, s \in \{ 0,1 \}^k  \quad s.t.  \quad X_s  \geq \eps \right)\\
			& \leq \sum_{ U \in \mathcal{U}_{\mathsf{Adv}}} \sum_{s \in \{ 0,1 \}^k} \Pr\left(  X_s  \geq \eps  \right) \\
			& \leq \sum_{ U \in \mathcal{U}_{\mathsf{Adv}}} \sum_{s \in \{ 0,1 \}^k} \sum_{j \in \{ 0,1 \}^k \ne s}  \Pr\left(  X_{js}  \geq \frac{\eps}{K}   \right) \\
			& \leq  | \mathcal{U}_{\mathsf{Adv}} | K^2 \Pr\left(  X_{js}  \geq \frac{\eps}{K}   \right) \\
			& \leq \mathcal{O} \left(\dfrac{K^2 N}{2^{N^{\alpha}}}\right) &(\mbox{from Eq.~\eqref{e1eq4}}). & \qedhere \\
		\end{align*}		
\end{proof}



\subsection*{From relaxed tamper detection to non-malleability}\label{Sec:nmcodes}
The relaxed form of tamper detection aims to either output the original message, or detect that it was tampered (indicated by the output $\perp$).
On the other hand, a non-malleable code insists that we either output the original message or an unrelated message, but with an additional requirement that the  probability (of a message being the same) depends only on the adversarial unitary $U$.
And hence, it is not a priori clear if relaxed tamper detection will immediately give non-malleable security.
In particular, the probability distribution may depend on $U$, as well as the original message $s$.
However, this potential dependency on $s$ can be removed by first analysing the distribution for an average $s$.
Then, a standard average-case to worst-case reduction shows that non-malleability can be achieved by incurring a nominal hit in the parameters.
This line of argument of first going to an average case setting to remove the dependency on $s$, followed by a reduction to worst case non-malleability is fairly common~(see for example, Section 3.3 in~\cite{BGJR23}). We include it below.


\begin{claim}\label{claimr:average_relaxed_TD}
Let $(\enc,\dec)$ be $\eps$-secure relaxed tamper detection scheme.
    Let $S$ be the uniform distribution on $\mathcal{M} = \lbrace 0,1 \rbrace^{k}$.
    Then, \[\dec \left( U \left( \enc(S)  \enc(S)^\dagger \right) U^\dagger  \right) \approx_{2 \eps} p_U S + (1-p_U)\perp,\]
    where $p_U= \frac{1}{2^k} \sum_s X_{ss}$.
\end{claim}
\begin{proof}
Note that, since $S$ is the uniform distribution,  each $s$ is sampled with probability $\frac{1}{2^k}$, and moreover, any particular $s$ gives back the same $s$ on decoding with probability $p_{\textsf{same}}(s)$, some different $s'$ with $p_{\textsf{diff}}(s)$ and $\perp$ with probability $p_{\perp}(s)$.
And hence, we can represent the relevant distribution as the following convex combination:
\[\dec \left( U \left( \enc(S)  \enc(S)^\dagger \right) U^\dagger  \right) = \frac{1}{2^k} \sum_{s} p_{\textsf{same}}(s) S + \frac{1}{2^k} \sum_{s} p_{\textsf{diff}}(s) S' + \frac{1}{2^k} \sum_{s} p_\perp(s) \perp.\]
Since $(\enc,\dec)$ is $\eps$-secure relaxed tamper detection code, $p_{\textsf{diff}}(s) \leq \eps$, for all $s$.

\noindent Thus, $\frac{1}{2^k} \sum_{s} p_{\textsf{diff}}(s) \leq \eps$.
The claim now follows by noting that $p_{\textsf{same}(s)} = X_{ss}$.
\end{proof}


\begin{theorem} \label{thm:non-malleability}
 Let $\mathcal{U}_{\mathsf{Adv}}$ be an $\left(N, \alpha, 1\right)$ family such that $ \left( \frac{1}{6} - \alpha\right) \log(N)  \geq 2\log(K) + \log\left( \frac{1}{\eps}\right)+ 5$. Then a uniform Haar random encoding-decoding strategy $(\enc,\dec)$ is a $2\eps$-secure non-malleable code (for classical messages against $\mathcal{U}_{\mathsf{Adv}}$) with probability at least $1-  \mathcal{O} \left(\dfrac{K^2 N}{2^{N^{\alpha}}}\right)$.
\end{theorem}
    \begin{proof}
Let $p_U = \frac{1}{2^k} \sum X_{ss}$ and $\eta = \perp$.
Set $\eps^\prime \leftarrow  \frac{\eps}{K}$\,.

\noindent Then, by choice of parameters, 
 $ \left( \frac{1}{6} - \alpha\right) \log(N)  \geq  \log(K) + \log\left( \frac{1}{\eps^\prime}\right)+ 5$.
 Hence, by Theorem~\ref{thm:relaxedclassical}, a Haar random encoding-decoding is $\eps^\prime$-secure relaxed tamper detection code with probability at $1- \mathcal{O}\left( \frac{K^2 N}{2^{N^{\alpha}}} \right)$.
Furthermore, by Claim~\ref{claimr:average_relaxed_TD}, 
\begin{equation}\label{eq:average_rtd_in_nonmalleability}
    \dec \left( U \left( \enc(S)  \enc(S)^\dagger \right) U^\dagger  \right) \approx_{2 \eps^\prime} p_U S + (1-p_U)  \perp \,.
\end{equation}
Now,
\begin{flalign*}
    & \Vert \dec \left( U \left( \enc(s)  \enc(s)^\dagger \right) U^\dagger  \right) - p_U s + (1-p_U) \perp\Vert_1 \\   \leq ~ & 2^k \cdot \Vert \dec \left( U \left( \enc(S)  \enc(S)^\dagger \right) U^\dagger  \right) - p_U S + (1-p_U) \perp\Vert_1 \\
     \leq ~ & 2^k \cdot 2 \eps^\prime & \hspace{1.236cm} (\mbox{from Eq.~\eqref{eq:average_rtd_in_nonmalleability}})  \\
     \leq ~ &  2 \eps \,.  &  \qedhere 
\end{flalign*}
    \end{proof}



  

==> TD/June_30_2023.tex <==




\input{TD/intro}
\input{TD/preliminaries}
\input{TD/classical_TD}
\input{TD/quantum_TD}
\input{TD/conclusion}

\begin{subappendices}

\input{TD/amd}

\newpage 

\section{Higher moments for classical messages \label{sec:app_classical}}
	%\begin{changemargin}{-0.123cm}{-0.123cm}
	Similar to the case of the first-order moments, we start expressing $X_{js}$ as a sum of products. 
We then deal with both the cases $j=s$ and $j \neq s$ individually. 
	    \input{TD/t_moments_classical}
	%\end{changemargin} 
	
	\newpage
 
    \section{Higher moments for quantum messages \label{sec:app_quantum}}
    
	%\begin{changemargin}{-0.123cm}{-0.123cm}
	We start by representing $X_m^t$ as a sum of products and then move on to calculating higher moments.
	
	    \input{TD/t_moments_quantum}
	%\end{changemargin}

\end{subappendices}

